Estimating global charge violating amplitudes from wormholes

We consider the scattering of high energy and ultra relativistic spherically symmetric shells in asymptotically AdS$_D$ spacetimes. We analyze an exclusive amplitude where a single spherically symmetric shell goes in and a single one comes out, such that the two have different global symmetry charges of the effective gravity theory. We study a simple wormhole configuration that computes the square of the amplitude and analyze its properties.

==> sec_junction.tex <==
\section{The junction conditions } \label{sec:junc}
 
 \YC{It seems that appendix A is also about junction condition}
 
 We can derive the junction conditions by looking at the equations of motion for the total action $I_{\rm grav} + I_{\rm shell}$ in the vicinity of the shell. These are easier to obtain in conformal gauge for the metric $g_{\mu \nu} = \eta_{\mu \nu} e^{ 2 \hat \omega}$. For a shell along $x^0$ in these coordinates the relevant terms near the shell are 
 \be \la{Actc}
 - I_t \sim  \int dx^0 dx^1 {   s \over 2 \pi } (-\partial^2 \hat \omega)  - \int dx^0 m(s) e^{\hat \omega} 
 \ee 
 giving the equations 
 \be \la{jumc}
 { 1 \over 2 \pi }  \partial_{1} \hat \omega |^+_-  + \partial_s m(s)e^{\hat \omega} =0~,~~~~~~~~~ { 1 \over 2 \pi } \partial_{ 1} s |^+_-  + m(s) e^{\hat \omega} =0
 \ee 
where $\pm$ indicate the two sides of the shell. We can covariantly write these as in \nref{JunCov}. 

The first equation in \nref{jumc} implies also a delta function in the curvature localized at the shell. When we integrate the action this leads to 
and extra term of the form  
\begin{equation} \la{CurvDel}
	\int \sqrt{g}\,\frac{s}{4\pi} \left( - 2 \nabla^2 \hat \omega\right) = \int dx^1\, e^{\hat \rho} s\partial_s m(s) =  \int d\ell \, s\partial_s m(s).
\end{equation}

\YC{I changed the conformal factor from $\rho$ to $\omega$ since we are using $\rho$ for the radial coordinate.}
